WeVibe: Weight Change Estimation Through Audio-Induced Shelf Vibrations In Autonomous Stores

Weight change estimation is crucial in various applications, particularly for detecting pick-up and put-back actions when people interact with the shelf while shopping in autonomous stores. Moreover, accurate weight change estimation allows autonomous stores to automatically identify items being picked up or put back, ensuring precise cost estimation. However, the conventional approach of estimating weight changes requires specialized weight-sensing shelves, which are densely deployed weight scales, incurring intensive sensor consumption and high costs. Prior works explored the vibration-based weight sensing method, but they failed when the location of weight change varies. In response to these limitations, we made the following contributions: (1) We propose WeVibe, a first item weight change estimation system through active shelf vibration sensing. The main intuition of the system is that the weight placed on the shelf influences the dynamic vibration response of the shelf, thus altering the shelf vibration patterns. (2) We model a physics-informed relationship between the shelf vibration response and item weight across multiple locations on the shelf based on structural dynamics theory. This relationship is linear and allows easy training of a weight estimation model at a new location without heavy data collection. (3) We evaluate our system on a gondola shelf organized as the real-store settings. WeVibe achieved a mean absolute error down to 38.07g and a standard deviation of 31.2g with one sensor and 10% samples from three weight classes on estimating weight change from 0g to 450g, which can be leveraged for differentiating items with more than 100g differences.

==> 05_Discussion.tex <==
\section{Discussions on WeVibe's Limitation and Future Work}
\label{sec:Limitations of WeVibe}
The amount of elastic deformation of the shelf surface might bring extra variation on the shelf vibration response, leading to more data collection on some specific locations. WeVibe performs worse at some locations such as location 1 shown in Figure~\ref{fig:Evaluation1} and location 5 shown in Figure~\ref{fig:Evaluation Real}. At these locations, some more weight classes are required to provide better estimation. It is probably because that there is a little amount of elastic deformation happened on these locations when the item weight changes, leading to more variances of the final weight change estimation.

On the other hand, WeVibe's weight change estimation does not work for one location while the weight at the other location changes. If the weight changes at location 1, for example, the whole structure of the shelf changes as well, influencing the vibration patterns across all locations, not just where the weight change occurred. This interdependency between multiple locations introduces complexity in accurately isolating the impact of weight changes at the area occupied by the same type of item, particularly in densely stocked shelves.

Therefore, to address these challenges, we would like to incorporate our vibration physics-informed model with existing sensing modality in the future. Integrating complementary technologies such as camera could significantly enhance the precision and reliability of WeVibe. By leveraging camera, we can provide real-time visual confirmation of item movements and weights, continuously updating and refining our weight estimation model to account for the elastic deformation. Furthermore, camera is also helpful on collecting weight samples with more various item layouts on the shelf, allowing us to do a more rigorous empirical study on the relationship between item weight on a single shelf and vibration response. Compared with item weight changes at different locations on the shelf, considering one shelf as "one" location is more compelling in the real-world scenario.

